Dissecting Continual Learning a Structural and Data Analysis

Continual Learning (CL) is a field dedicated to devise algorithms able to achieve lifelong learning. Overcoming the knowledge disruption of previously acquired concepts, a drawback affecting deep learning models and that goes by the name of catastrophic forgetting, is a hard challenge. Currently, deep learning methods can attain impressive results when the data modeled does not undergo a considerable distributional shift in subsequent learning sessions, but whenever we expose such systems to this incremental setting, performance drop very quickly. Overcoming this limitation is fundamental as it would allow us to build truly intelligent systems showing stability and plasticity. Secondly, it would allow us to overcome the onerous limitation of retraining these architectures from scratch with the new updated data. In this thesis, we tackle the problem from multiple directions. In a first study, we show that in rehearsal-based techniques (systems that use memory buffer), the quantity of data stored in the rehearsal buffer is a more important factor over the quality of the data. Secondly, we propose one of the early works of incremental learning on ViTs architectures, comparing functional, weight and attention regularization approaches and propose effective novel a novel asymmetric loss. At the end we conclude with a study on pretraining and how it affects the performance in Continual Learning, raising some questions about the effective progression of the field. We then conclude with some future directions and closing remarks.

==> chapters/papers/unsup/abstract.tex <==
\begin{abstract}
    Unsupervised image segmentation is a well-defined problem only when dealing with syntactic features. This is the case, for instance, when seeking for objects of similar colors or areas separated by sharp edges. When semantic comes into play, things become more and more slippery, as the binding between low-level appearance and segments is lost. Supervised methods would solve the issue by building a statistical model of the relevant objects to be segmented, being them people, trees or cars. Unsupervised approaches, by contrast, would need to automatically learn the models, however it is not clear which should be the implicit definition of an ``object'', neither how to set the correct hierarchical segmentation level, which can range from a tree as a whole to a single leaf.
    With this paper we try to solve this quandary in the special (but not uncommon) scenario where several complete or partial repetitions of similar subjects are found in the scene. The leading idea is that if a pattern is replicated consistently enough it has good chances of being a well defined object from a semantic standpoint.  
    Specifically, we introduce a fast algorithm to find, without any supervision, hierarchical visual categories from repeated similar pattern in images. In order to assess the quality of a segmentation spanning different levels of detail we introduce the notion of ``semantical levels'' and we devise a conceptual framework along with metrics and a dedicated benchmark dataset. The effectiveness of our method is then measured by performing both qualitative and quantitative experimental validations.

\end{abstract}

==> chapters/papers/unsup/abstract_pelosin.tex <==
\begin{abstract}
    We propose a new fast fully unsupervised method to discover semantic patterns. Our algorithm is able to hierarchically find visual categories and produce a segmentation mask where previous methods fail. Through the modeling of what is a visual pattern in an image, we introduce the notion of ``semantic levels'' and devise a conceptual framework along with measures and a dedicated benchmark dataset for future comparisons. Our algorithm is composed by two phases. A filtering phase, which selects semantical hotsposts by means of an accumulator space, then a clustering phase which propagates the semantic properties of the hotspots on a superpixels basis. We provide both qualitative and quantitative experimental validation, achieving optimal results in terms of robustness to noise and semantic consistency. We also made code and dataset publicly available.

\keywords{visual-pattern-detection  \and semantic-discovery \and cosegmentation}
\end{abstract}


==> chapters/papers/unsup/introduction_pelosin.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
%                            INTRODUCTION
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5

\section{Introduction}
\label{sec:introduction}

The extraction of semantic categories from images is a fundamental task in image understanding \cite{mottaghi2014role,cordts2016cityscapes,zhou2017scene}. While the task is one that has been widely investigated in the community, most approaches are supervised, making use of labels to detect semantic categories \cite{chen2018encoder}. Comparatively less effort has been put to investigate automatic procedures which enable an intelligent system to learn autonomously extrapolating visual semantic categories without any \textit{a priori} knowledge of the context. 

We observe the fact that in order to define what a visual pattern is, we need to define a scale of analysis (objects, parts of objects etc.). We call these scales \textit{semantic levels} of the real world. Unfortunately most influential models arising from deep learning approaches still show a limited ability over scale invariance \cite{singh2018analysis,li2019scale} which instead is common in nature. In fact, we don't really care much about scale, orientation or partial observability in the semantic world. For us, it is way more important to preserve an ``internal representation'' that matches reality \cite{DiCarlo2012HowDT,logothetis1996visual}.


\begin{figure}[t]
  \centering
  \includegraphics[width=1\linewidth]{figures/levels.jpg}
  \caption{A real world example of unsupervised segmentation of a grocery shelf. Our method can automatically discover both low-level coherent patterns (brands and logos) and high-level compound objects (detergents) by controlling the semantic level of the detection and segmentation process.}
  \label{fig:levels}
\end{figure}


Our method leverages repetitions (Figure \ref{fig:levels}) to capture the internal representation in the real world and then extrapolates categories at a specific semantic level. We do this without continuous geometrical constraints on the visual pattern disposition, which is common among other methodologies \cite{DBLP:conf/cvpr/PrittsCM14,DBLP:conf/cvpr/PrittsCM14,DBLP:conf/wacv/LettryPVG17,DBLP:journals/cg/Rodriguez-Pardo19,DBLP:conf/cvpr/HeZRS16}. 

We also do not constrain ourselves to find only one visual pattern, which is another very common assumption. Indeed, what if the image has more than one visual pattern? One can observe that this is \textit{always} the case. Each visual repetition can be hierarchically decomposed in its smaller parts which, in turn, repeat over different semantic levels. This peculiar observation allow our work to contribute to the community as follows:

\begin{itemize}
    \item A new pipeline able to capture semantic categories with the ability to hierarchically span over semantic levels.
    \item A better conceptual framework to evaluate analogous works through the introduction of the semantic levels notion along with a new metric.
    \item A new benchmark dataset of 208 labelled images for visual repetition detection. 
\end{itemize}

Code, dataset and notebooks are public and available at:  \texttt{\url{https://git.io/JT6UZ}}.



==> tables/more_is_better/cifar100.tex <==


\begin{tabular}{@{}ccc@{}}
\toprule
\multicolumn{3}{c}{\textbf{CIFAR100}} \\
\textit{Method} & \textit{Acc@3MiB} & \textit{Acc@6MiB} \\ 
\midrule
AGEM \cite{agem} & 9.05 $\pm$ 0.4 & 9.3 $\pm$ 0.4 \\
ER \cite{DBLP:conf/nips/RolnickASLW19} & 11.02 $\pm$ 0.4 & 14.6 $\pm$ 0.4 \\
EWC \cite{kirkpatrick_overcoming_2017} & 4.8 $\pm$ 0.2 & 4.8 $\pm$ 0.2 \\
GSS  \cite{gss} & 9.3 $\pm$ 0.2 & 10.9 $\pm$ 0.3 \\
ER-MIR \cite{aljundi2019online} & 11.2 $\pm$ 0.3 & 14.1 $\pm$ 0.2 \\
ASER \cite{shim2020online} & 12.3 $\pm$ 0.4 & 14.7 $\pm$ 0.7 \\
ASER$_{\mu}$ \cite{shim2020online} & 14.0 $\pm$ 0.4 & 17.2 $\pm$ 0.5 \\
\rowcolor{red!15}
GDumb \cite{prabhu2020greedy} & 17.1 $\pm$ 0.2 & 25.7 $\pm$ 0.7 \\
\bottomrule
\rowcolor{orange!15}
Resize (8x8) & \textbf{38.5 $\pm$ 0.4} & \textbf{? $\pm$ ?} \\
\rowcolor{blue!20}
ELM (128) & \textbf{22.4 $\pm$ 0.3} & \textbf{25.7 $\pm$ 0.3} \\
\rowcolor{green!20}
CutR (8x8) & \textbf{32.6 $\pm$ 0.6} & ? $\pm$ ?
\\ \bottomrule
\end{tabular}


==> tables/more_is_better/imagenet100.tex <==


\begin{tabular}{@{}ccc@{}}
\toprule
\multicolumn{3}{c}{\textbf{ImageNet100}} \\
\textit{Method} & \textit{Acc@12MiB} & \textit{Acc@24MiB} \\ 
\midrule
AGEM \cite{agem} & 7.0 $\pm$ 0.4 & 7.1 $\pm$ 0.5 \\
ER \cite{DBLP:conf/nips/RolnickASLW19} & 8.7 $\pm$ 0.4 & 11.8 $\pm$ 0.9 \\
EWC \cite{kirkpatrick_overcoming_2017} & 3.2 $\pm$ 0.3 & 3.1 $\pm$ 0.3 \\
GSS  \cite{gss} & 7.5 $\pm$ 0.5 & 10.7 $\pm$ 0.8 \\
ER-MIR \cite{aljundi2019online} & 8.1 $\pm$ 0.3 & 11.2 $\pm$ 0.7 \\
ASER \cite{shim2020online} & 11.7 $\pm$ 0.7 & 14.4 $\pm$ 0.4 \\
ASER$_{\mu}$ \cite{shim2020online} & 12.2 $\pm$ 0.8 & 14.8 $\pm$ 1.1 \\
\rowcolor{red!15}
GDumb \cite{prabhu2020greedy} & 10.0 $\pm$ 0.? & 21.6 $\pm$ 0.3 \\
\bottomrule
%\rowcolor{blue!15}
GDumb (Resize+ResNet) & \textbf{20.0.? $\pm$ 0.?}  & - \\
%\rowcolor{green!20}
GDumb (ELM) & \textbf{13.3 $\pm$ 0.2}  & 15.4 $\pm$ 0.4 \\
%\rowcolor{yellow!20}
GDumb (CutR+ResNet) & \textbf{??.? $\pm$ 0.?} & - \\ 
\bottomrule
\end{tabular}



==> titlepage.tex <==
\makeatletter
\begin{titlepage}
	
	\includegraphics[width=3.5cm]{unive_logo}
	
	\begin{center}
		
		\vspace*{1cm}
		
		{\Large Ph.D. Thesis % change Master with Bachelor if you're a BSc normie
			
			34$^{th}$ Cycle (D.M. 270/2004) in % don't change this line
			\vspace*{0.2cm} % otherwise the next line isn't properly spaced, dunno why lel
			
			Computer Science}
		
		\vspace*{0.75cm}
		
		%{\Large Final Thesis}
		
		\vspace*{0.75cm}
		
		{\LARGE\bfseries \@title} % write it by hand if you want fancy new lines
		
	\end{center}

	\vfill 

\begin{flushright}
		\noindent\textbf{Supervisor}\\
	Prof. Andrea Torsello
	
	\vspace*{0.55cm}
	
	\noindent\textbf{Graduand}\\
	\@author
\end{flushright}
	
	\vspace*{0.25cm}
	
	\noindent\textbf{Academic Year}\\
	2021-22
	
\end{titlepage}
\makeatother
